HungerGist: An Interpretable Predictive Model for Food Insecurity

The escalating food insecurity in Africa, caused by factors such as war, climate change, and poverty, demonstrates the critical need for advanced early warning systems. Traditional methodologies, relying on expert-curated data encompassing climate, geography, and social disturbances, often fall short due to data limitations, hindering comprehensive analysis and potential discovery of new predictive factors. To address this, this paper introduces "HungerGist", a multi-task deep learning model utilizing news texts and NLP techniques. Using a corpus of over 53,000 news articles from nine African countries over four years, we demonstrate that our model, trained solely on news data, outperforms the baseline method trained on both traditional risk factors and human-curated keywords. In addition, our method has the ability to detect critical texts that contain interpretable signals known as "gists." Moreover, our examination of these gists indicates that this approach has the potential to reveal latent factors that would otherwise remain concealed in unstructured texts.

==> 01_introduction.tex <==
\section{Introduction}

% food crisis prediction: significance, current methods, data efforts
Africa has been increasingly vulnerable to food insecurity due to factors such as drought, climate change, conflict, and poverty. In 2022, one of five people in Africa are in danger of acute hunger impacting over 140 millions of Africans \cite{ReliefWeb_2022}. An early estimate of food crisis prediction is in need to predict probability of impending shocks and maps of risk for each region. Such systems are known to help identify vulnerable areas and effectively target resources to areas of greatest need \cite{Extremeclimateeventsincreaserisk, endtoendassessmentextremeweatherimpacts}, as well as to improve socioeconomic and political stability \cite{buhaug2021vicious, martin2019food}.

% statistical factors
A number of studies have shed light on the various statistical factors that can be utilized to predict food insecurity, including food supply and availability, climates, or agricultural factors \cite{MeasuringHouseholdFoodInsecurityWhy, Extremeclimateeventsincreaserisk, endtoendassessmentextremeweatherimpacts}. Food insecurity has previously been studied at the fine-grained level, such as the availability and utilization of food in households \cite{MeasuringHouseholdFoodInsecurityWhy}. Later, researchers began to examine the macro-level factors such as climate changes or agricultural aspects including droughts, precipitation, crop growth, vegetation index, land usage, and terrain ruggedness \cite{datadrivenapproachimprovesfoodinsecurity, forecastabilityfoodinsecurity, krishnamurthy2022anticipating}.

% more factors, one by one
Among those factors, socio-economic elements are viewed as important as other non-social elements (e.g., agricultural factors) -- in particular, social factors such as international aid, population density, government corruption, economy, and urbanization have been accounted to have a major effect on the food crisis \cite{FoodsecurityconflictEmpiricalchallenges,Violentconflictexacerbateddroughtrelatedfood, WarConflictFoodInsecurity, ArmedConflictsFoodInsecurityEvidence}.

Understanding the complex interactions between the various factors affecting food insecurity in African countries can be critical for anticipating future food crises and preparing resources for crisis mitigation. However, existing work have heavily relies on the availability of data from various sources, traditionally presumed to impact food crises, spanning climate, geography, and social conflicts. Yet, these data sources, primarily collected by NGOs, often lack real-time updates, constraining our ability to forecast food crises promptly. Because of the limitations of the data at hand, studies that rely on such conventional factors can never fully account for all possible influences. This also prevents us from expanding our pre-existing knowledge and exploring what other factors might improve food crisis prediction.

This study seeks to bridge these gaps by harnessing news texts and the NLP techniques to propose potential solutions for improving food crisis prediction. Among efforts of recent studies to leverage various types of big data, a recent study paid attention to leveraging news articles, typically published on a day-to-day basis and available for up-to-date information. Using large-scaled news corpus, they conducted ad-hoc text analysis using techniques such as topic modeling or keyword statistics \cite{PredictingFoodCrises}. While such analysis sheds light on uncovering previously unknown predictive associations, not accessible through predefined features, the approach tends to heavily hinge on a complex pipeline to process a large pool of candidate texts into useful features, requiring labor-intensive efforts and insights from experts.

In this paper, we introduce \name, a multi-task deep learning classifier for both predictive and interpretable food insecurity. We pay attention to the nature of food crisis influenced by multidimensional factors evidenced from previous studies, and leverages them as multiple objectives of a multi-task classifier known as better predictive by learning mutually associated tasks and optimizing better latent representation, in our case, including three critical objectives: food price, social instability, and food insecurity. Furthermore, our approach is inherently interpretable, providing ``gist'' for predicting ``hunger'' crisis, the most critical contexts and events drawn from a vast amount of texts, with textual evidence signaled as highly predictive of a high or low likelihood of food insecurity across various topics at both sentence and phrase level. Our analysis is based on the corpus of 56,065 news articles collected from GDELT Project\footnote[2]{GDELT is a database covers news media in over 100 languages across print, broadcast, and web formats, from almost every corner of each country, on a constant, everyday basis.}, covering nine African countries including  Uganda, Guinea, Malawi, Mali, Niger, Nigeria, Senegal, Burkina Faso, and Democratic Republic of the Congo over four years (between 2017 and 2020). This dataset was further expanded using a bootstrapping method to cope with data scarcity in spatial-temporal data, a potential issue happening even in large-scaled data. We show that our analysis outperforms the baseline predictor trained from both traditional factors and textual features \cite{PredictingFoodCrises}, showing better predictive capabilities of food insecurity only with news corpus. Furthermore, our qualitative analysis on important textual features reveals phrases from news articles that are highly predictive of high or low food crises across various topical factors, demonstrating our model’s capacity to identify latent factors. Our contributions can be summarized as follows: (1) We propose a method called bootstrap data augmentation, which addresses the challenge of data scarcity happening due to uneven distribution of data across country-month contexts. This approach provides a useful strategy for food crisis analysis to cope with a lack of observations from spatial-temporal contexts. (2) We present \name, an interpretable predictive model engineered for achieving both food insecurity prediction and enhanced interpretability. Our model, trained solely on news data, outperforms the baseline predictor and has the unique capability to provide sentence-level evidence that predicts food insecurity. Our study highlights the potential of data-driven ways of assisting decision-makers in government and private sector in comprehending complex socioeconomic factors and formulating policies to address them effectively.




==> 030_problem_old.tex <==
\section{Problem Statement}
Let there be $C$ countries, each represented by a set of features $X$. 
There are static features $S_{c} \in X$ that remain the same across time for each country $c \in C$, for instance population. 
There are also dynamic features such as rainfall, noted as $D_{c, m} \in X$, vary from month to month. 
We note the time ticks at month level as $m \in M$.
For each country and month, we collect the news articles from the internet as textual features $T_{c, m} \in X$.
The target variable of food insecurity index $Y_{c,m} \in [1, 5]$ is given as real numbers. 
Our goal is to predict a future food crisis index $Y_{m}$ with the data of the previous month $m-1$.
Therefore, our objective can be formulated as learning an optimal function $f(S_{c}, D_{c, m-1}, T_{c, m-1}) \rightarrow Y_{c, m}$ that maps the features to the prediction of crisis index.

In the next sections, we will introduce the detailed features inside $X$, and the model we develop for the prediction.

% Y per month per country
% k Articles A
% F features


% \yrl{Before this section, need a section for "Problem Statement". One important information to provide here is the unit of analysis (country rather than district, monthly, quarterly, or yearly) and the scale of the features (dynamic vs static)}

==> 032_baseline.tex <==
\subsection{Baseline Model}

\begin{figure*}[h]%
\centering
\small
\includegraphics[width=0.7\textwidth]{figures/model.pdf}
\caption{The deep neural architecture of interpretable multi-task classifier for predicting food insecurity.}
\label{fig:teaser}
\end{figure*}

To assess the predictive performance, we compare HungerGist with a baseline model presented in \cite{Finegrainedpredictionfoodinsecurityusing}\footnote{Note that the model published in \cite{Finegrainedpredictionfoodinsecurityusing} was replicated as the baseline model of our paper at the time of our study development. Later, the same researcher published an updated version of the model -- with a random forest model trained on quarterly observations. In our paper, this baseline model remains on a monthly basis to facilitate the comparison, but we report the experiment results with random forest}. In the paper, xx et al. developed a machine learning approach to leverage both a corpus of news articles as well as data for traditional features outlined in Section \ref{sec:data-traditional}. Both types of features are collectively integrated into a panel autoregressive distributed lag (ADL) model, enabling to incorporate both time-lagged temporal factors and time-invariant factors within the analysis.

Specifically, the baseline predictor consists of four parts: (1) self-lagged target features for three to eight months, (2) five time-varying features with three to eight months of lagged values, and (3) time-invariant features. Among them, time-varying features include nine traditional factors listed in Table \ref{tab:data} and textual features from news data. We first incorporate textual features as frequencies of a list of keywords discovered in \cite{Finegrainedpredictionfoodinsecurityusing}.

We train the baseline models using cross-validation on split data. We partitioned the observational months into 10 periods as folds that progressively span recent months. Within each fold, we subsequently segmented the data into training, validation, and testing subsets using a temporal split.


==> 033_bootstrap.tex <==
\subsection{Bootstrap Data Augmentation}


Our dataset is composed of a large body of texts in news reports and a small number of monthly food crisis labels.
It results in a ``wide data'' where we have significantly more features than the number of samples.
This creates challenges for deep neural network models (to be introduced next in Section~\ref{sec_034:multi-task-model}) as the models are easily overfit the data.
We apply bootstrap sampling on the raw data to augment the data with more samples.

Let $A = \{s_1, s_2, ... s_n\}$ represent an article with $n$ sentences.
For each country-month tuple, there are $k$ articles articles $m = \{A_1, A_2, ... A_k\}$.
And for each month, there is one corresponding label, that is, the food-crisis label of the next month, represented as $Y_m$.
Our goal is to re-sample $k$ articles $\hat{m} = \{\hat{A_1}, \hat{A_2}, ... \hat{A_k}\}$ for each month $m$, and each re-sampled article is consisted with $i$ bootstrapped sentences from the sentence pool of that month.

In this experiment, we use the median number of sentences of each article $n = 21$, and the median number of articles of each month $k = 85$.
Each month-country tuple is one data sample in the prediction task, and it contains 85 articles bootstrapped.
We implement the bootstrap re-sampling 10 times and eventually get 9 (countries) $\times$ 44 (months) $\times$ 10 (bootstrap folds) = 3960 samples containing 336600 (3960 $\times$ 85) bootstrapped articles after the augmentation.

==> 034_multitask.tex <==
\subsection{Multi-task Modeling} \label{sec_034:multi-task-model}

% Why multi-task
While we fine-tune the deep model utilizing the language signals to produce latent feature representations for predicting the \fews, the information from related prediction targets can potentially further optimize the learned representations.
There is a technique of using side-task prediction to improve the target-task prediction performance, named multi-task learning, and it is proven to be effective in various domains \cite{XX}. 
Food price and social unrest have been repeatedly mentioned when studying food insecurity \cite{XX}. 
It is arguable that signals that are predictive tho these two variables are also informative to the food insecurity prediction.
We add the prediction task of those two variables in addition to the \fews prediction, and let the three prediction tasks utilize the same set of learned latent representation, so that the model can potentially perform better on the \fews prediction from the multi-task learning.


We employ a multi-task attention neural network to predict \fews with the collection of articles per country-month as input.
The attention layer adopts the Dot-product attention layer structure \cite{luong2015effective}.
Let $\vec{h_i} \in \mathcal{R}^d$ be the embedded vector for article $i$ in a country-month tuple (such a tuple makes a sample for the prediction task), there is a dense attention layer that outputs the attention weight for each given $\vec{h_i}$ as:

\begin{equation}
    w_i = \vec{h_i}\vec{a} + b
\end{equation}

where the $\vec{a} \in \mathcal{R}^{d \times 1}$ is the attention layer weight and $b$ is the scalar bias.
The collection of embedded articles of each country-month tuple ${\vec{h_1}, \vec{h_2}, ... \vec{h_k}}$ is then weight-summed as:

\begin{equation}
    \vec{h_{all}} = \sum_{1}^{k} w_i\vec{h_i}
\end{equation}


The attention output is then fed to three distinct dense layers for a multi-task prediction.

\begin{equation}
    \hat{y}_{task} =  dense(\vec{h_{all}})
\end{equation}

Where $dense(\cdot)$ is a single-task dense layer outputting the prediction value $\hat{y}_{task}$ from the joint hidden representation $\vec{h_{all}}$ of all articles of a certain country-month tuple.
Specifically, in this study, we include three tasks: the \fews, the food price, and social insecurity event number prediction.

For each of these three tasks, the regression output is compared with the true value for computing a MSE loss.

\begin{equation}
    loss_{task} = \sum({\hat{y}_{task} - y_{task}})^2
\end{equation}

The total loss of the model is the equally weighted sum of all three losses.

\begin{equation}
    loss = loss_{fci} + loss_{fp} + loss_{si}
\end{equation}

where $fci$ denote \fews, $fp$ denote Food Price and $si$ denote Social Insecurity.




==> 040_results.tex <==
\section{Results}

\input{041_predictions}
\input{042_attentions}

==> 041_predictions.tex <==
\input{tables/regression_results_yrl}

\subsection{Food Crisis Prediction}

As summarized in Table \ref{tab:regression_results}, we report our experiment results on predictive performance in Root Mean Square Error (RMSE). We also provide a summary of the performance of four different model variants, each with different sets of objectives, referred to as single- (solely predicting food insecurity), dual- (additionally predicting food price or social security), and triple-tasks (considering all three objectives). Overall, the results indicate that our model achieves better overall prediction across nine countries than the baseline predictor relying on the combination of traditional and keyword-based features. Especially, our full model leads to a drop in RMSE to 26\% (1.074 $\rightarrow$ 0.790). We observe that our analysis represents a significant step towards data-driven approaches, reducing the efforts required for both data collection and feature extraction compared to the baseline predictors, which involve extensive manual preprocessing steps.

We also observe that there is variability in prediction results at country-level performance. In most countries, our full model achieves better RMSE compared to other model variants; Nevertheless, in Guinea and Senegal, a dual model, tasked with food and social insecurity, obtained better RMSE than the full model, indicating lower efficacy of food prices additionally involved in the full model in specific contexts. Also, in Niger and Burkina Faso, the baseline predictor achieved better predictive performance than our model variants. This suggests that while our models, trained exclusively on news data, demonstrate competitive performance, the instability of food consumption in certain countries could be significantly influenced by traditional factors, which implies the necessity of taking various factors into account in specific contexts when analyzing food insecurity.



==> 042_attentions.tex <==
\subsection{Attention Weight Analysis}

We rank the sentences on the calculated $w_s$ (as described in Section~\ref{sec_034:multi-task-model}) to identify sentences associated with high or low \fews for the following qualitative analysis.

\input{figures/fig01}
\subsubsection{Topic Analysis of High-importance Sentences}
We use topic model to comprehensively summarize the characteristics of sentences corresponding to high and low ${w_s}$.
We use Mallet LDA \cite{graham2012getting} to model the topics among the whole corpus.
The texts are lemmatized and stopwords are removed before the model training.
We discovered eight topics in total, and manually named them according to the top keywords of each topic.
The topics are: Food Price, Leadership, Regional Development, Finance, Land Scale, Economic Development, Health Care, and Civil Life.
The trained topic model is used to infer the topic probability for the sentences. 
We sum the topic probability distribution of top 5\% sentences with the highest $w_s$ and that of bottom 5\% sentences, as shown in Figure~\ref{fig:topic}.

While the Land Scale topic distributes similarly in high and low \fews sentences, there are noticeable differences in other topic distributions between the two categories.
Sentences corresponding to lower \fews tend to have a higher portion in Finance and Economic Development topics. 
This confirms our previous qualitative analysis.
On the other hand, sentences corresponding to higher \fews tend to be more related to Food Price and Health Care topics.




\input{figures/fig02}
\subsubsection{Semantic Differences of Topical Texts between High and Low Crisis Index}

We report example sentences that correlate the most with high and low \fews grouped by topics in Figure~\ref{fig:examples}.
% Different from the manual analysis presented earlier in this section, the samples are extracted from the top-ranked ones from the deep learning model, grouped by the learned topics. 
% The examples are ranked by the model attention weights 


There is a clear tendency that the texts often report ``good’’ events when being more informative to predict a low crisis index and vice versa. 
Specifically, for the topic ``Food Supply’’, the example reports positive fertilizer application rates for peanut farms, which compose a signal in the deep learning model to predict a low crisis index outcome. 
On the other hand, within the same topic, the example reports investigations on a massive death of fishes. 
Similarly, for the topic ``Politics/Leadership’’, political figures’ announcement on peaceful reconciliation corresponds to a low crisis index, while a report related to election polling fraud predicts a high food crisis. 
Lastly, in ``Healthcare’’, the national budget funding healthcare section is informative to a low crisis index prediction, and a health crisis caused by delayed social assistance is important to a high crisis prediction.
This adds evidence that the model is capable of discovering meaningful news events that correlate with food crisis predictions in Africa.


In sum, in this section, we employ qualitative analysis on the attention weights of the \fews prediction tasks, and discover textual content characteristics that correspond to the predicted scores.


==> 050_discussion.tex <==
\section{Discussion and Conclusion}
\label{sec:discussion}

In this study, we presented \name, an interpretable predictive model for food insecurity analysis. We demonstrated that our multi-task deep classifier, tasked with simultaneously predicting three critical objectives (food insecurity, food price, and social insecurity) not only improves food crisis prediction but also enhances interpretable, as evidenced by our experiment results and analysis. In contrast to prior work \cite{forecastabilityfoodinsecurity, PredictingFoodCrises, gholami2022food}, our model inherently provided interpretability with sentence-level evidence from texts. We showed in the qualitative analysis that top-associated sentences span across diverse topics such as food supply, politics/leadership, and healthcare, and are indicative of food insecurity either to a lower (e.g., the use of fertilizer increasing crop production, reconciliation among different leaderships) or higher (e.g., electoral fraud, health crisis) degree. When aggregated, these sentences yielded quantifiable and diverse insights spanning eight distinct topics. 

From the analysis perspective, our approach supports an efficient analysis pipeline, simplifying the data collection process by relying solely on news articles, which can be less time-consuming to collect compared to traditional data sources. In the analysis stage, interpretability can be readily achieved through a data-driven approach by quantifying scores derived from the model, eliminating the need for laborious processing steps or expert insights. Moreover, our approach facilitates the discovery of diverse latent factors not available from explicitly encoded features, as demonstrated in our topic analysis.

To provide support in mitigating real-world food crises, our analysis has potential to advance the development of automatic monitoring tools. We expect that organizations and decision makers at governments or public sectors could benefit from establishing a monitoring process without the extensive data curation and feature extraction efforts. As mentioned earlier, the monitoring is not restricted to the availability of data sources, but can adapt to capture emerging or hidden factors, thus enhancing the ability to respond to ever-changing circumstances due to local and global events such as covid-19 pandemic \cite{falkendal2021grain}.

However, our approach has certain limitations. While our analysis was conducted at the country level, a finer-grained level of analysis (e.g., at the district-level) might better capture the variability of the food crisis happening at local areas. Our analysis can be adapted to use at various spatial-temporal levels with available data. To perform the analysis at a finer-grained level, some heuristics, such as identifying mentions or news sources as indicators of specific spatial units of interest, could be employed to process in a data-driven manner. Furthermore, our analysis can be extended to incorporate traditional features to further enhance both predictive performance and interpretability. As discussed earlier, different types of features from various sources have been proven to increase the forecastability of food crises, thus are in need of efforts to consistently develop ways to collectively integrate variables into analysis to respond to the complex and multidimensional nature of food insecurity.

==> 88_ref.tex <==
\section*{References}

Please number citations consecutively within brackets \cite{b1}. The 
sentence punctuation follows the bracket \cite{b2}. Refer simply to the reference 
number, as in \cite{b3}---do not use ``Ref. \cite{b3}'' or ``reference \cite{b3}'' except at 
the beginning of a sentence: ``Reference \cite{b3} was the first $\ldots$''

Number footnotes separately in superscripts. Place the actual footnote at 
the bottom of the column in which it was cited. Do not put footnotes in the 
abstract or reference list. Use letters for table footnotes.

Unless there are six authors or more give all authors' names; do not use 
``et al.''. Papers that have not been published, even if they have been 
submitted for publication, should be cited as ``unpublished'' \cite{b4}. Papers 
that have been accepted for publication should be cited as ``in press'' \cite{b5}. 
Capitalize only the first word in a paper title, except for proper nouns and 
element symbols.

For papers published in translation journals, please give the English 
citation first, followed by the original foreign-language citation \cite{b6}.

\begin{thebibliography}{00}
\bibitem{b1} G. Eason, B. Noble, and I. N. Sneddon, ``On certain integrals of Lipschitz-Hankel type involving products of Bessel functions,'' Phil. Trans. Roy. Soc. London, vol. A247, pp. 529--551, April 1955.
\bibitem{b2} J. Clerk Maxwell, A Treatise on Electricity and Magnetism, 3rd ed., vol. 2. Oxford: Clarendon, 1892, pp.68--73.
\bibitem{b3} I. S. Jacobs and C. P. Bean, ``Fine particles, thin films and exchange anisotropy,'' in Magnetism, vol. III, G. T. Rado and H. Suhl, Eds. New York: Academic, 1963, pp. 271--350.
\bibitem{b4} K. Elissa, ``Title of paper if known,'' unpublished.
\bibitem{b5} R. Nicole, ``Title of paper with only first word capitalized,'' J. Name Stand. Abbrev., in press.
\bibitem{b6} Y. Yorozu, M. Hirano, K. Oka, and Y. Tagawa, ``Electron spectroscopy studies on magneto-optical media and plastic substrate interface,'' IEEE Transl. J. Magn. Japan, vol. 2, pp. 740--741, August 1987 [Digests 9th Annual Conf. Magnetics Japan, p. 301, 1982].
\bibitem{b7} M. Young, The Technical Writer's Handbook. Mill Valley, CA: University Science, 1989.
\end{thebibliography}

==> tables/regression_results.tex <==
\begin{table*}[]
\centering
\caption{\label{tab:regression_results} \textbf{Regression Results.}}
\begin{tabular}{@{}lccccc@{}}
\toprule
 &
  \multicolumn{1}{l}{\textbf{Baseline}} &
  \multicolumn{1}{l}{\textbf{Single Task}} &
  \multicolumn{1}{l}{\textbf{Double-task with Food Price}} &
  \multicolumn{1}{l}{\textbf{Double-task with Social Insecurity}} &
  \multicolumn{1}{l}{\textbf{Triple-task}} \\ \midrule
All          & 0.874 & 0.819 & 0.841 & 0.827 & 0.79  \\
Burkina Faso & 1.827 & 0.942 & 1.018 & 0.987 & 0.94  \\
Congo        & 1.483 & 1.036 & 1.04  & 1.036 & 0.949 \\
Guinea       & 1.96  & 0.418 & 0.444 & 0.412 & 0.548 \\
Malawi       & 1.268 & 0.667 & 0.704 & 0.769 & 0.662 \\
Mali         & 1.463 & 1.041 & 1.096 & 0.995 & 0.982 \\
Niger        & 1.871 & 1.066 & 1.125 & 0.999 & 1.058 \\
Nigeria      & 2.03  & 0.538 & 0.459 & 0.564 & 0.403 \\
Senegal      & 1.285 & 0.331 & 0.37  & 0.337 & 0.452 \\
Uganda       & 1.631 & 0.914 & 0.862 & 0.961 & 0.798 \\ \bottomrule
\end{tabular}
\end{table*}
